Learning-Based Animation of Clothing for Virtual Try-On

This paper presents a learning-based clothing animation method for highly efficient virtual try-on simulation. Given a garment, we preprocess a rich database of physically-based dressed character simulations, for multiple body shapes and animations. Then, using this database, we train a learning-based model of cloth drape and wrinkles, as a function of body shape and dynamics. We propose a model that separates global garment fit, due to body shape, from local garment wrinkles, due to both pose dynamics and body shape. We use a recurrent neural network to regress garment wrinkles, and we achieve highly plausible nonlinear effects, in contrast to the blending artifacts suffered by previous methods. At runtime, dynamic virtual try-on animations are produced in just a few milliseconds for garments with thousands of triangles. We show qualitative and quantitative analysis of results

==> 0-abstract.tex <==
\begin{abstract}


This paper presents a data-driven method to produce detailed clothing animations at interactive frame rates. Our method is built upon standard skinning techniques, which we use to obtain an approximate model of the garment's motion. We then enhance this model by introducing a vector of corrective offsets that are computed by a recurrent neural network (RNN). In order to obtain realistic animations, the network learns these offsets from physically simulated sequences. We show that our method solves some of the visual limitations of previous works and is capable of generating plausible results in unseen motions. Moreover, our method can be easily integrated into existing skeletal animation pipelines with little computational overhead.

\end{abstract}


\begin{CCSXML}
    <ccs2012>
    <concept>
    <concept_id>10010147.10010371.10010352.10010379</concept_id>
    <concept_desc>Computing methodologies~Physical simulation</concept_desc>
    <concept_significance>500</concept_significance>
    </concept>
    <concept>
    <concept_id>10010147.10010257.10010293.10010294</concept_id>
    <concept_desc>Computing methodologies~Neural networks</concept_desc>
    <concept_significance>500</concept_significance>
    </concept>
    </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computing methodologies~Physical simulation}
\ccsdesc[500]{Computing methodologies~Neural networks}



\keywords{Cloth simulation, data-driven simulation, machine learning, neural networks}


